Attention Distillation: A Unified Approach to Visual Characteristics Transfer

Recent advances in generative diffusion models have shown a notable inherent understanding of image style and semantics. In this paper, we leverage the self-attention features from pretrained diffusion networks to transfer the visual characteristics from a reference to generated images. Unlike previous work that uses these features as plug-and-play attributes, we propose a novel attention distillation loss calculated between the ideal and current stylization results, based on which we optimize the synthesized image via backpropagation in latent space. Next, we propose an improved Classifier Guidance that integrates attention distillation loss into the denoising sampling process, further accelerating the synthesis and enabling a broad range of image generation applications. Extensive experiments have demonstrated the extraordinary performance of our approach in transferring the examples' style, appearance, and texture to new images in synthesis. Code is available at https://github.com/xugao97/AttentionDistillation.

==> _paper.tex <==

\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
    \vspace{-1\baselineskip}
    \includegraphics[width=\linewidth]{figs/teaser_final.pdf}
     \captionof{figure}{Given a reference image, our approach can faithfully reproduce its visual characteristics in synthesis, providing a unified framework for a wide range of example-based image synthesis applications, such as artistic style transfer, appearance transfer, style-specific text-to-image generation, and various texture synthesis tasks.}
    \vspace{1em}
    \label{fig:teaser}
\bigskip}

\makeatother


\maketitle
\input{sec/0_abstract}    
\input{sec/1_intro}
\input{sec/2_related}
\input{sec/3_method}
\input{sec/4_exp}
\input{sec/5_con}

\section*{Acknowledgments}
This work was supported in parts by NSFC (U21B2023), ICFCRT (W2441020), Guangdong Basic and Applied Basic Research Foundation (2023B1515120026), Shenzhen Science and Technology Program (KQTD20
210811090044003, RCJC20200714114435012, KJZD20
240903100022028), and Scientific Development Funds from Shenzhen University.

{
    \small
    \bibliographystyle{ieeenat_fullname}
    \bibliography{main.bib}
}

==> sec/0_abstract.tex <==
\begin{abstract}
Recent advances in generative diffusion models have shown a notable inherent understanding of image style and semantics. 
In this paper, we leverage the self-attention features from pretrained diffusion networks to transfer the visual characteristics from a reference to generated images. Unlike previous work that uses these features as plug-and-play attributes, we propose a novel attention distillation loss calculated between the ideal and current stylization results, based on which we optimize the synthesized image via backpropagation in latent space. Next, we propose an improved Classifier Guidance that integrates attention distillation loss into the denoising sampling process, further accelerating the synthesis and enabling a broad range of image generation applications. Extensive experiments have demonstrated the extraordinary performance of our approach in transferring the examples' style, appearance, and texture to new images in synthesis.  Code is available at \url{https://github.com/xugao97/AttentionDistillation}.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
% Task and application

Synthesizing new images with visual elements, such as the style or texture, of an example image, is a long-standing yet challenging problem in computer graphics and vision.
The key challenge lies in properly representing images' texture or style features. 
Traditional methods~\cite{Efros:2001, kwatra2003, kwatra2005, patchmatch, imagemelding, PG15, Self-tuning, EG17} usually define textures as repeated local patterns and synthesize new textures by copying local patches from the source image.
When it comes to style, an extensive yet more abstract visual characteristic than texture, new representations are required. 

Thanks to the deep learning revolution, neural representations of visual features have emerged. One group of approaches performs texture or style-specific synthesis by matching the global distribution of deep features between the reference and the output. For example, the seminal work Gram loss~\cite{Gatys2015, gaty2016styletransfer} regards the feature maps' statistics as the texture/style representation. Some other work optimizes deep features by minimizing Wassertein distance~\cite{heitz2021sliced} or adversarial discrimination loss~\cite{TexExp,shaham2019singan, InGAN}. However, matching global distributions lacks local perception, usually leading to conspicuous detail artifacts. Another group retakes the local patch strategy, optimizing output's deep features through nearest-neighbor matching~\cite{LiChuanandWand2016, mechrez2018contextual, zhou2023neural}. As local patches are unaware of global structure, these methods always require additional structural guidance.

%methods for texture synthesis and style transfer. Now, content and style are deriving not only from images but also from textual descriptions, thus significantly enhancing creative possibilities while introducing new challenges. 

Beyond the above progress, recent breakthroughs in large-scale diffusion models have sparked new representations for visual features, reaching a good balance between global and local consistency in synthesis~\cite{cao2023masactrl, hertz2024stylealigned, jeong2024visual, alaluf2024cross, chung2024styleid, zhou2024generating}. 
A key consensus of these techniques is that the \emph{keys} ($K$) and \emph{values} ($V$) from the self-attention module of pretrained diffusion models characterize the appearance of the exemplar. Re-aggregating these features according to target \emph{queries} ($Q$) by self-attention mechanism during new image generation can reproduce the visual characteristics of the reference. Although impressive results were achieved due to the robust performance of diffusion models, these methods still often suffer issues like insufficient stylization. We hypothesize three reasons for their limitations:

1) \emph{Domain gap}. When two images differ significantly, the similarity between the target $Q$ (queries of the synthesized image) and the source $KV$ (keys and values of the exemplar) will become low and unreliable, leading to erroneous aggregation results. Techniques like AdaIN~\cite{AdaIn} and attention scale can partially mitigate this issue~\cite{hertz2024stylealigned, alaluf2024cross}.

2) \emph{Error accumulation}. While the iterative sampling process in diffusion models can ameliorate large discrepancies between the target $Q$ and the source $KV$, errors may also accumulate. As demonstrated in~\cite{tang2023emergent}, features from different layers of diffusion models focus on distinct information, such as semantics and geometry. Incorrect matches will propagate errors to subsequent layers along the Markov chain and degrade the final image quality.

%\emph{Error accumulation}. While the iterative sampling process in diffusion models can ameliorate large discrepancies between the target Q and the source KV, it may also accumulate errors, degrading the final image quality. %is chain-like, with dependencies between layers and time steps. While this process
 %is chain-like, with dependencies between layers and time steps. While this process

3) \emph{Architectural limit}. The self-attention mechanism is implemented within the residual branch of the denoising network. Injecting self-attention features from the source may have a bounded influence on the target latent code, potentially diminishing their efficacy in the synthesis.

%(queries of the generated image) (keys and values of the examplar)
In this work, we still follow the assumption that the self-attention features in the denoising networks capture an image's visual appearance. To address the above-mentioned limitations, we introduce a novel \emph{Attention Distillation} (AD) loss, based on which we directly update the synthesized image through backpropagation. Specifically, we consider the output obtained by computing the attention between the target $Q$ and the source $KV$ as the \emph{ideal} stylized result, and the original attention output represents the current stylization. We define attention distillation loss as the L1 distance between these two outputs and optimize the synthesized image through backpropagation in latent space. We simultaneously calculate the differences across various layers to avoid error accumulation. Such an optimization process gradually reduces the disparity between the target $Q$ and the source $KV$, enhancing the accuracy of similarity calculations and thus improving the final stylization.

Whereas our approach differs greatly from previous works that use self-attention features as plug-and-play attributes, the new attention distillation loss can also be integrated into the sampling process of diffusion models, functioning as an \emph{improved Classifier Guidance}. Combined with the normal Classifier-Free Guidance, it further enables text-based controlled generation, and is also compatible with other conditioning technologies such as ControlNet, leading to broad image synthesis applications; see, \eg, Fig.~\ref{fig:teaser}. Extensive experiments and comparisons with state-of-the-art methods have demonstrated our advantages. %in various example-based style or texture synthesis tasks. 

In summary, our main contributions are as follows:
\begin{itemize}
    \item We analyze the limitations of previous plug-and-play attention features methods and propose a novel attention distillation loss for reproducing the visual characteristics of a reference image, achieving notably superior results.  %compared to existing approaches.
    \item We develop attention distillation guided sampling, an improved Classifier Guidance that integrates attention distillation loss into the denoising process, which significantly accelerates synthesis speed and enables a wide range of visual characteristics transfer and synthesis applications. %Combined with normal Classifier-Free Guidance, it enables text-based controlled generation and is also compatible with other technologies such as ControlNet and IP-Adapter, demonstrating a wide range of applications.
\end{itemize}



%Texture synthesis and style transfer represent significant and challenging research areas within computer vision and computer graphics. 
%Texture synthesis aims to generate similar and continuous images that share visual characteristics with a given reference texture. Neural style transfer, initially proposed by Gatys et al.\cite{gaty2016styletransfer}, seeks to transfer the style of one image onto another while preserving the content, thus creating novel artistic works. Style transfer can be viewed as an extension of texture synthesis, and both techniques have extensive applications in image processing, artistic creation, and the film and gaming industries.

% Technical challenge for previous methods (围绕我们解决了的technical challenge展开讨论。Technical challenge包括limitation和technical reason)
%such as Gram matrix loss, histogram loss, sliced Wasserstein distance loss, and adversarial loss optimize parameters by minimizing the distributional discrepancy between synthesized and example images. These methods perform well in general texture synthesis and style transfer. Nevertheless, they 
%like CNNMRF and Contextual loss, utilize pretrained VGG, a classification network, to extract features, seeking the nearest neighbors for each pixel or patch in feature space, with Euclidean distance or similarity as the optimization objective. 
%Deep learning-based texture synthesis and style transfer algorithms typically rely on well-defined loss functions as supervisory signals to optimize model parameters through backpropagation. However, existing losses often struggle to achieve a satisfactory balance between global and local consistency. Distribution matching losses~\cite{gaty2016styletransfer, li2017demystifying, risser2017stable, heitz2021sliced, shaham2019singan} lack semantic correspondence, often resulting in unreasonable synthesis when handling semantic style transfer or non-stationary textures. Nearest-neighbor matching losses\cite{LiChuanandWand2016, mechrez2018contextual}, leveraging the semantic information from deep neural networks, significantly enhance semantic style transfer. However, they often neglects global distributional consistency. When applied to texture synthesis, these methods frequently produce noticeable repetition. Furthermore, the VGG network's inherent limitations in semantic understanding impede accurate semantic matching when content and style images differ substantially.

%Recent years have witnessed breakthrough advancements in diffusion models for image generation, sparking widespread interest among researchers. This progress has led to the flourishing of diffusion model-based techniques for style transfer and texture synthesis. The scope of style transfer has expanded, now deriving content and style not only from images but also from textual descriptions, thus significantly enhancing creative possibilities while introducing new challenges. 
%One category of these methods employs KV-injection\cite{cao2023masactrl, hertz2024style, jeong2024visual, alaluf2024cross, chung2024style, zhou2024generating} to maintain appearance or style consistency. These approaches extract keays (K) and values (V) of the exemplar from self-attention module in pretrained diffusion model. And re-aggregating these features by self-attention mechanism during new image generation to ensure visual consistency. Leveraging the robust performance of diffusion models, these methods have achieved impressive results. Nevertheless, they often suffer from insufficient stylization, necessitating additional techniques such as AdaIN, copying, shuffling of latents during sampling, or attention scale to enhance visual quality. We hypothesize three potential reasons for the limitations of these methods:

% 1) When the content and style images differ significantly, the similarity computed between Q from the synthesized image and K from the example image may be uniformly low, leading to erroneous aggregation results. Techniques like AdaIN and attention scale can partially mitigate this issue.

% 2) The sampling process in diffusion models is chain-like, with dependencies between layers and time steps. While this process can ameliorate large discrepancies between querys (Q) and keys (K), it may also accumulate errors, ultimately degrading image quality.

% 3) The self-attention mechanism's implementation within the residual branch of network limits the full potential of KV-injection. This architectural constraint impedes the complete manifestation of KV-injection's effects, potentially diminishing its efficacy in style transfer and texture synthesis tasks.

% 介绍解决challenge的our pipeline

%In this work, we introduce a novel style loss—attention distillation loss—based on KV-injection, ingeniously leveraging the model's attention mechanism. Through backpropagation, we directly apply the effects of KV-injection to the synthesized image, fully exploiting the potential of the attention mechanism. Utilizing the diffusion model's inherent understanding of image style and semantics, we achieve a balance between global and local consistency, resulting in optimal visual effects. Specifically, we extract image features from the self-attention module of a pretrained diffusion model. We consider the output obtained by computing attention between the querys (Q) from the generated image and the keys (K) and values (V) from the example image as the ideal stylized result, while the original attention output represents the unstylized result. We define the style loss as the L1 distance between these two outputs and optimize the synthesized image through backpropagation in latent space. This approach simultaneously calculates differences across various layers, avoiding error accumulation between layers and directly updating the synthesis result through backpropagation. The optimization process gradually reduces the disparity between Q and K, enhancing the accuracy of similarity calculations and ultimately yielding the desired visual effect.

% In summary, our main contributions are as follows:
% \begin{itemize}
%     \item We propose a novel attention distillation loss, overcoming the stylization limitations of traditional KV injection methods and achieving superior results in texture synthesis and style transfer tasks compared to existing approaches.
%     \item We develop an Improved Classifier Guidance method that integrates attention distillation loss into the model sampling process, accelerating synthesis speed. This method, combined with Classifier-Free Guidance, enables text-based controlled generation and is compatible with technologies such as ControlNet and IP-Adapter, demonstrating broad application prospects.
% \end{itemize}

% Experiment
% Contributions

% \yangc{Below are useless texts...}

% Image style transfer and texture synthesis have emerged as compelling applications within the domain of computer vision, enabling the transformation of images by adopting stylistic features from other sources. Traditionally, techniques such as the Gram Matrix have been utilized to capture style representations, facilitating the synthesis of new images that blend content with desired aesthetics. However, recent advancements in neural architectures, particularly diffusion networks, have revealed significant limitations in these conventional methods. 

% Diffusion networks operate on the principle of progressive denoising, allowing for nuanced image generation through iterative refinement. Yet, when integrating Gram Matrix-based style representations, we have observed a pronounced discrepancy in performance. The inherent characteristics of diffusion networks—namely their reliance on attention mechanisms—remain underexplored in the context of style transfer, leading us to question the adequacy of established representations for these modern models.

% In this work, we propose a novel style representation derived from the attention mechanisms within diffusion networks. By leveraging attention maps, which capture the relationships and importance of different image regions, we can create a more adaptive and context-aware representation of style. This approach not only addresses the shortcomings of previous techniques but also aligns more closely with the operational dynamics of diffusion networks. Our methodology allows for richer texture synthesis and more compelling style transfer results by effectively harnessing the intricacies of attention.

% Furthermore, we conduct a series of experiments to demonstrate the efficacy of our proposed representation. We compare its performance against traditional methods, providing qualitative and quantitative analyses that highlight its advantages. Our findings indicate that attention distillation not only enhances the visual quality of generated images but also offers greater flexibility in manipulating styles, paving the way for more sophisticated applications in digital artistry.

% Ultimately, this research contributes to a deeper understanding of how attention mechanisms can be utilized in creative tasks, bridging the gap between theoretical exploration and practical application. We envision that our work will inspire further innovations in image processing, setting a foundation for future studies that seek to integrate advanced neural architectures with artistic creativity.




%Recent advancements in texture synthesis and style transfer methods based on optimization have yielded significant results. These methods typically utilize pre-trained networks, such as VGG, to extract features for calculating well-defined style losses, such as the Gram matrix and sliced Wasserstein distance. Through gradient descent methods, they continuously update and optimize the pixel values of the images. These losses are often defined based on the distance between two distributions. Notably, different pre-trained networks can influence the effectiveness of these losses, as demonstrated in a study exploring the use of ResNet for style transfer.
%Currently, diffusion models have showcased remarkable capabilities in image generation and editing, particularly with the open-source nature of the Stable Diffusion series, which has spurred rapid advances in AI-assisted art. This raises an important question: can the previously defined style losses be effectively applied to the Stable Diffusion model? Furthermore, is there a suitable style loss specifically tailored for this model?
%Drawing on the lessons from using ResNet in style transfer, our objective is to identify an appropriate style loss for the Stable Diffusion model. Recently, a plethora of research based on Self-KV has emerged, leveraging self-attention features (KV) from U-Net in Stable Diffusion as a plug-and-play attribute to maintain consistency in appearance or style. The consensus in the research community is that utilizing Self-KV is an effective way to ensure visual coherence. Given the challenges in directly applying traditional style and texture synthesis losses to Stable Diffusion, we propose a straightforward and effective loss function grounded in Self-KV, enabling style transfer and texture synthesis in the latent space of Stable Diffusion.


\label{sec:intro}


==> sec/2_related.tex <==
\section{Related work}
\label{sec:related_work}

Our primary contribution lies in proposing a novel loss function that effectively transfers the visual characteristics of one image to another. This loss function has broad applications across various image synthesis tasks, including texture synthesis, style transfer, appearance transfer, and customized image generation based on text-to-image models. We review related work in these domains.

\textbf{Texture synthesis} focuses on generating images that resemble the original texture without repetition and artifacts. Traditional methods rely on parametric texture models~\cite{Julesz, Heeger_Bergen_1995, Simoncelli_Freeman_2002} or sampling pixels/patches~\cite{Efros_Leung_1999, Wei_Levoy_2000, Efros:2001, kwatra2003, kwatra2005} to create new images.
%Early parametric models, like the multiscale model by Portilla and Simoncelli (2000), generate textures by matching the statistical properties of the target texture image. Non-parametric approaches, such as Efros and Leung’s (1999) sample-based synthesis algorithm, generate new images pixel-by-pixel or block-by-block, leveraging previously synthesized regions to produce natural texture effects. 
%Although these methods excel with simple textures, they often struggle with complex or high-resolution textures.
These methods excel with simple textures but often struggle with complex or high-resolution textures.
Deep learning-based methods, utilizing convolution neural networks (CNNs), extract multilevel features that capture textures at varying scales. Gatys~\etal~\cite{Gatys2015} introduced Gram matrix, a second-order statistic of feature map to represent stationary textures.
%a CNN-based texture synthesis approach, using Gram loss to match feature statistics between input and target textures. However, Gram loss primarily captures second-order statistics, which may inadequately represent complex textures. 
Histogram loss~\cite{risser2017stable} and Sliced Wasserstein loss~\cite{heitz2021sliced, elnekave2022generating} offer improved modeling of texture distributions, leading to more realistic results but failing to capture large-scale structure, especially for non-stationary textures. Generative adversarial networks (GANs) are also widely adopted in texture synthesis~\cite{TexExp, shaham2019singan, InGAN}; for instance, Zhou~\etal~\cite{TexExp} used a self-supervised approach to expand a single texture by learning the internal patch distribution, achieving impressive detail and structure expansion. Recently, Self-Rectification~\cite{zhou2024generating} leverages pre-trained diffusion networks and the self-attention mechanism to gradually refine a lazy-editing input, addressing the intricate challenge of synthesizing non-stationary textures.

%extracts content and style features through a VGG network,
\textbf{Neural style transfer} %an extension of texture synthesis in the arts, 
applies the artistic style of a source image to a new content image. Gatys~\etal~\cite{gaty2016styletransfer} pioneered this field by using Gram loss as style representation and proposed a neural style transfer algorithm that combines content and style loss in the optimization. While Gram loss and its variants~\cite{Johnson2016, AdaIn, li2017demystifying} are the most widely used style losses, they primarily assess global distribution differences and cannot account for local semantic correspondences. Approaches like CNNMRF~\cite{LiChuanandWand2016} and Contextual Loss\cite{mechrez2018contextual} address this by computing semantic similarity in high-dimensional feature spaces to enable semantically coherent style transfer. %To accelerate the optimization process, a generative network is introduced for a real-time style transfer~\cite{Johnson2016}. Subsequently, Huang~\etal~\cite{AdaIn} proposed adaptive instance normalization (AdaIN), enabling arbitrary style transfer in real-time. 
Later works incorporated transformers with self-attention to capture stronger relationships between style and content. Deng~\etal~\cite{Deng_Tang_Dong_Ma_Pan_Wang_Xu_2022} introduced a fully transformer-based architecture, StyTR$^2$, achieving state-of-the-art results at the time. Recent advances in diffusion models enable interpretable and controllable content-style separation. InST~\cite{zhang2023inst} proposed inversion-based learning of artistic style from a single painting.  StyleDiffusion~\cite{wang2023stylediffusion} introduced a CLIP-based style disentanglement loss. StyleID~\cite{chung2024styleid}, a training-free method, manipulates the self-attention features of a pre-trained diffusion model by substituting the keys and values of the content with those of the style image in cross-attention mechanisms.


\textbf{Appearance transfer}, a specialized semantic style transfer, aims at transferring the appearance of semantically corresponding regions. Early works~\cite{Isola_Zhu_Zhou_Efros_2017, Zhu_Park_Isola_Efros_Winter_Gogh_Monet_Photos, Park_Zhu_Wang_Lu_Shechtman_Efros_Zhang_2020} use paired or unpaired datasets to train GANs for domain-specific appearance transfer. Tumanyan~\etal~\cite{Tumanyan_Bar-Tal_Bagon_Dekel_2022} extract structure and appearance features using a pre-trained DINO-ViT~\cite{Caron_Touvron_Misra_Jegou_Mairal_Bojanowski_Joulin_2021}, and trains a generator for each image pair. Recently, cross-image attention~\cite{alaluf2024cross} with pre-trained diffusion models realizes zero-shot appearance transfer by implicitly establishing semantic correspondences across images.

% with text
\textbf{Customized/Personalized image generation} based on text-to-image (T2I) diffusion models has attracted particular attention recently, which aims to learn the style from one or more reference images to generate new content. 
%\textbf{Diffusion models}~\cite{ho2020denoising, song2021ddim,dhariwal2021beatgans,esser2024sd3, Podell2023SDXLIL,Rombach2021HighResolutionIS} have recently demonstrated groundbreaking capabilities in text-to-image (T2I) generation, significantly advancing related fields. 
%Customized (or personalized) style generation based on T2I models has attracted particular attention, aiming to learn the style from one or more reference images to generate new content. 
Fine-tuning approaches~\cite{ahn2024dreamstyler, everaert2023diffusioninstyle, frenkel2024implicit, Gal2022AnII, jones2024customizingtexttoimagemodelssingle, kumari2022customdiffusion, Ruiz2022DreamBoothFT, sohn2023styledrop} enable models to learn novel style concepts from a few images. However, these methods are prone to overfitting, potentially resulting in degraded image quality or content leakage. To alleviate this issue, B-LoRA~\cite{frenkel2024implicit} leverages LoRA~\cite{hu2022lora} (Low-Rank Adaptation) to implicitly separate the style and content components of a single image. Pair Customization~\cite{jones2024customizingtexttoimagemodelssingle} learns stylistic differences from a single image pair and then applies the acquired style to the generation process. Encoder-based methods~\cite{ye2023ip-adapter, xing2024csgo, gao2024styleshot,chen2023controlstyle, wang2024styleadapter, wang2024instantstyle} utilize visual encoders to capture image information and establish mappings between image prompts and models through huge dataset training. While currently favored as state-of-the-art, these techniques are constrained by the capabilities of visual encoders, often extracting only abstract style information and struggling with fine-grained textures of the reference. Several works have proposed plug-and-play solutions for training-free style customization. For example, StyleAligned~\cite{hertz2024stylealigned} and Visual Style Prompt~\cite{jeong2024visual} maintain style consistency by preserving the queries from the original features while sharing or swapping the keys and values with those from reference features in the late self-attention layers. RB-Modulation~\cite{rout2024rbmodulation} modulates the drift field of reverse diffusion dynamics by incorporating desired attributes (\eg, style or content) through a terminal cost.

% \subsection{Neural Style Transfer}
%  The seminal work of Gatys \etal~\cite{Gatys2016} reveals that deep features extracted from pretrained VGG networks encode the content information of an image, while statistics computed from activation maps of different scales can represent the image style. An image then can be modified via back-propagation by matching the disentangled representations of content and style features with those of the reference. The impressive stylization results produced by this method have popularized neural style transfer and inspired a surge of successive works, including training feed-forward networks~\cite{Johnson2016, AdaIn}, combining with Markov Random Fields~\cite{LiChuanandWand2016}, and utilizing multi-scale strategies~\cite{WCT, ETNet} etc. \yangc{Describe the drawbacks of Gatys' method here, e.g.,} \yang{However, the capacity of convolution neural networks limits its representation power. In this work, we opt to diffusion networks and propose new representations for both content and style.}

% Gatys' pioneering work and impressive results have led people to explore new methods for style transfer and texture synthesis in the feature space of VGG. Gram loss and histogram statistics minimize the distance between the distributions of two images by calculating the statistical differences between them, while SWD directly computes the differences between the distributions of two images using sliced Wasserstein distance. The GAN-based SinGAN essentially aligns the distribution of generated images with that of real images through a discriminator. We categorize these methods as distribution-based styling approaches, which have a global optimization objective but lack semantic correspondence (e.g., eye-to-eye, mouth-to-mouth).\par
% On the other hand, approaches like CNNMRF, contextual loss, and GCD search the nearest neighbors (pixels or image patches) based on similarity within the VGG feature space to serve as optimization targets, leveraging VGG's recognition capabilities to establish semantic correspondence. We refer to these as semantic-based styling methods. However, since the VGG network is trained on the ImageNet dataset for classification tasks, its performance is limited in understanding higher-level abstract semantics in style images. When there is a lack of semantic correspondence between the content and style images (e.g., Picasso's bull and a human face), these methods often fail to achieve the desired stylistic effects.\par
% These losses often emphasize the correspondence of semantic or the similarity of distributions, failing to capture the essence and nuances of the original work.
% In this paper, we argue that the pretrained Stable Diffusion model can be likened to a highly skilled artist, adept at extracting both low-level visual elements and high-level semantic information from reference images. This virtuoso then, drawing upon its vast reservoir of experience (akin to the attention mechanism), ingeniously recombines these elements into novel creations. Through our innovative loss function, we succeed in distilling the entirety of this artist's expertise and knowledge, capturing the essence of the example artworks .

 

% \subsection{T2I diffusion models and personalization}
% Recent advancements in T2I diffusion models, particularly within the Stable Diffusion series \cite{esser2024sd3, Podell2023SDXLIL,Rombach2021HighResolutionIS}, have significantly enhanced the quality and diversity of images generated from textual prompts. The release of the Stable Diffusion community model has further broadened its impact, fostering a more extensive adoption and exploration. T2I personalization using Stable Diffusion has attracted considerable attention, with efforts focusing on incorporating new concepts into these models. Some approaches \cite{alaluf2023neti, Gal2022AnII, voynov2024p} introduce new textual embeddings to encapsulate the unique characteristics of the desired content, while others \cite{hao2024vico, hua2023dreamtuner, kumari2022customdiffusion, marjit2023diffusekrona, pang2024attndreambooth, Ruiz2022DreamBoothFT, Ruiz2024hyperdreambooth, shah2023ZipLoRA} modify or append specific model parameters to achieve personalized outputs. Although effective in generating personalized and concept-specific images, these approaches often struggle with maintaining consistent text alignment and fully capturing the complexity of intricate styles.
% %学习来自图像的新概念， create images consistent in style, subject, or character ID
% %基于微调的方法：dreambooth TI LoRA，3-5张图像
% %基于图像编码器的方法：IP Adapter InstantID 人脸个性化是目前的一个热门研究方向
% %kv特征注入:masactrl magicface 


% \subsection{Style-specific image generation} 
% Style transfer in T2I generation has been a prominent area of research. Starting with the traditional style transfer \cite{gaty2016styletransfer}, which applying the artistic style of one image to the content of another, recent works \cite{chung2024styleid, he2024freestyle, wang2023stylediffusion, zhang2023inst} have advanced to using diffusion models. Another line of research is on custom style text-to-image generation. One approach \cite{ahn2024dreamstyler, everaert2023diffusioninstyle, frenkel2024implicit, Gal2022AnII, jones2024customizingtexttoimagemodelssingle, kumari2022customdiffusion, Ruiz2022DreamBoothFT, sohn2023styledrop} involves fine-tuning models on style-specific image data, while another features training-free methods, such as StyleAligned \cite{hertz2024stylealigned}, RB-Modulation \cite{rout2024rbmodulation} and InstantStyle \cite{wang2024instantstyle}, which leverage pre-trained models to integrate styles without additional training. Additionally, there are pre-trained methods \cite{chen2023controlstyle, gao2024styleshot, wang2024styleadapter, xing2024csgo} designed to handle arbitrary styles, offering a versatile solution for style-specific image generation. However, fine-tuning methods often struggle with achieving desired style effects and can suffer from text-semantic loss. Training-free and pre-trained methods also face challenges when handling multiple style images as input.
% %基于T2I的风格迁移方法，可以看作T2I个性化在风格领域的一个子集，
% %微调的方法 InST TI DB-LoRA  可以很好的捕捉到图像的细节信息，但容易过拟合和内容泄露 B-LoRA缓解了上述问题，但只在SDXL上有效，这些方法通常也比较耗时
% %图像编码器：IPAdapter styleshot csgo instantstyle， 基于大数据训练，使编码器更容易捕捉到高层次的抽象风格信息，可能存在泛化性不足的问题，对于罕见的风格效果并不理想
% %kv特征注入：style aligned styleID vsp  无需训练，做到了即插即用，但有时效果并不理想。一是kv注入本身存在问题，二是该方法受到模型自身性能限制，masactrl以二次元动漫图作为参考图时选用了Anything-V4，一个使用二次元动漫数据集微调的模型，应该也是这个原因。目前来看，sd1.5对3d、二次元动漫等风格表现不佳，是因为训练数据没有包含太多这类数据，SDXL则有了很多适用的风格提示词，应该是做了特定的风格训练。
% Fine-tuning approaches, such as DreamBooth, Textual Inversion (TI), and InST, enable models to learn novel style concepts from one or more images. However, these methods are prone to overfitting, potentially resulting in degraded image quality or content leakage. Encoder-based methods utilize visual encoders to capture image information and establish connections between image prompts and models through vast datasets. While currently favored as state-of-the-art, these techniques are constrained by the capabilities of visual encoders, often extracting only abstract style information and struggling with complex texture details.

%我们的主要贡献是提出一种新的损失函数，能够有效地将参考图像中的视觉元素（如纹理风格）迁移到另一张图像上。这一损失可以广泛应用于多个计算机任务，例如纹理合成、风格迁移、外观迁移，以及基于文生图模型的特定风格图像生成。我们将回顾这些领域的相关工作。

%纹理合成专注于生成与原始纹理相似但不重复的图像，以模拟自然界中的无缝纹理。传统的纹理合成方法基于样本统计或样本拼接来生成新图像。最早的统计模型如Portilla和Simoncelli（2000）提出的基于参数化的多尺度模型，通过匹配目标纹理图像的统计特性来生成新纹理。非参数化方法则如Efros和Leung（1999）提出的基于样本的合成算法，通过逐像素或逐块生成新图像，每一步都依赖之前生成的像素或块的信息，以此生成自然的纹理效果。这类方法虽然在合成简单纹理上效果显著，但在复杂纹理或分辨率较高的场景下往往难以生成自然的纹理图像。基于深度学习的纹理合成方法通过卷积神经网络（CNN）从图像中提取多层次特征，这些特征在不同层中表现为不同的纹理尺度。Gatys等人（2015）首次提出了一种基于深度卷积网络的纹理合成方法，通过Gram Loss 优化输入图像的特征图，使其与目标纹理图像的统计特征匹配。然而Gram loss主要用于计算特征的二阶统计量，无法完全表示复杂纹理的统计分布。直方图损失和瓦瑟斯坦损失对纹理的特征分布进行更精准的建模，使生成的纹理更加逼真。但这些损失无法捕捉到纹理的大尺度结构，对于非稳态纹理的合成效果不佳，需要引入额外的控制。此外，生成对抗网络（GAN）在纹理合成中也被广泛使用，zhou等人设计了自监督的方式学习纹理扩展，利用GAN学习纹理的数据分布，在纹理细节和结构延伸上取得了令人满意的效果。最近Self-rectification leverages a pre-trained diffusion network, and uses self- attention mechanisms, to gradually refine a lazy-editing input, addressed the intricate challenge of synthesizing non-stationary textures
% 神经风格迁移作为纹理合成在艺术领域的扩展，可以视为在目标图像的内容特征上，应用源图像的纹理特征。Gatys等人（2016）提出的经典基于Gram loss的神经风格迁移算法是风格迁移领域的开创性工作，该算法使用VGG网络来提取图像的内容和风格特征，采用内容损失和风格损失的加权和作为目标函数。Gram loss及其变体MMD虽然是今天应用最为广泛的风格损失，但这种衡量数据全局分布差异的损失，无法consider局部的语义对应，CNNMRF、Contextual Loss等基于最近邻匹配的思想，在高维特征空间计算语义相似度，进而设计损失函数，实现了令人满意的语义风格迁移。另一方面，为解决优化过程较为耗时的问题，Johnson等人（2016）提出了基于生成网络的快速风格迁移方法，从而实现了实时风格迁移。此外，Dumoulin等人（2017）和Huang与Belongie（2017）分别提出了多风格迁移和自适应实例归一化（AdaIN），通过修改生成网络的参数或归一化方式实现多种风格迁移，使得风格迁移的应用更加灵活。
% 外观迁移，一种特别的语义风格迁移，旨在迁移语义对应区域的外观特征。早期的工作通过成对或非成对数据集训练GAN，实现特定域图像的外观迁移效果。Tumanyan et al. extract structure and style feature with a pretrained DINOVi and train a generator for each pair of images. Recently Cross image attention 借助预训练扩散模型implicitly establishes semantic correspondences across images。借助 a cross-image attention mechanism 实现了Zero-Shot Appearance Transfer。

%近年来，扩散模型凭借其优异的生成能力，在T2I领域取得突破性进展，并促进了相关领域的研究。其中风格定制化备受关注。
 

==> sec/3_method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/method1.pdf} 
    \caption{\textbf{Overview of attention distillation.} Based on the self-attention mechanism in diffusion models, we compute the difference between the ideal and the current stylization, formulating a novel Attention Distillation (AD) loss (a). The new loss acts like a style loss. When combined with a content loss (also derived from the self-attention mechanism), we can realize high-quality content-preserving synthesis, such as style transfer or appearance transfer (b). Our attention distillation loss can be incorporated into the normal diffusion sampling process as an improved Classifier Guidance (c), which enables a broad scope of example-based image generation applications.}
    \label{fig:method}
\end{figure*}

\section{Method}


\subsection{Preliminaries}
\textbf{Latent diffusion models (LDM)}, exemplified by Stable Diffusion~\cite{Podell2023SDXLIL,Rombach2021HighResolutionIS}, have achieved state-of-the-art performance in image generation due to the robust ability to model complex data distributions. In LDM, an image $x$ is first compressed into a learned latent space using a pretrained VAE $\mathcal{E}(\cdot)$. A UNet-based denoising network $\epsilon_\theta(\cdot)$ is subsequently trained to predict the noise during the diffusion process by minimizing the mean squared error between the predicted noise and the actually added noise $\epsilon$:
\begin{equation}
    \mathcal{L}_{\mathrm{LDM}}=\mathbb{E}_{z\sim\mathcal{E}(x),y,\epsilon\sim\mathcal{N}(0,1),t}\Big[\|\epsilon_\theta(z_t,t,y)-\epsilon\|_2^2\Big],
\end{equation}
where $y$ denotes the condition and $t$ represents the timestep. The denoising UNet typically consists of a bunch of convolution blocks and self-/cross-attention modules, all integrated within the predictive branch of \textit{residual} architecture.

\textbf{KV-injection} is widely employed in image editing~\cite{pnpDiffusion2022, cao2023masactrl, alaluf2024cross}, style transfer~\cite{hertz2024stylealigned, chung2024styleid, jeong2024visual}, and texture synthesis~\cite{zhou2024generating}. 
It is built upon the self-attention mechanism and uses the self-attention features in diffusion models as plug-and-play attributes. The self-attention mechanism is formulated as:
\begin{equation}
\mathrm{Self\text{-}Attn}(Q,K,V)=\mathrm{softmax}(\frac{QK^T}{\sqrt{d}})V.
\end{equation}
At the core of the attention mechanism lies the calculation of a weight matrix based on the similarity between the queries ($Q$) and keys ($K$), which is used to perform a weighted aggregation of the values ($V$). KV-injection extends this mechanism by copying or sharing the $KV$ features across different synthesis branches. Its key assumption is that $KV$ features represent the visual appearance of an image. During sampling, replacing the $KV$ features in the synthesized branch with those $KV$ from the corresponding timestep of the exemplar can realize appearance transfer from the source image to the synthesized target.
% However, direct feature injection during diffusion sampling is influenced by the residual mechanism, which limits its ability to fully leverage the potential of KV-injection. 

%Diffusion sampling with KV-injection refers to synthesizing images by drawing information from the KV features of the reference branch. However, it cannot fully capture the style or texture details from the reference due to the residual mechanism;

\subsection{Attention Distillation Loss}
\label{sec:method_ADL}
Although KV-injection has achieved noticeable results, it falls short in preserving the style or texture details of the reference due to the residual mechanism; see Fig.~\ref{fig:kvinjection}~(a) for example. KV-injection only operates on the residual, which means the information flow (red arrows) is subsequently influenced by the identity connection, leading to an incomplete transfer of information. As a result, the sampling outputs cannot fully reproduce the desired visual details.

%\yang{optimization} and sampling with .}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/kvinjection1.pdf} 
    % \vspace*{-3mm}
    \caption{\textbf{Differences between KV-injection and attention distillation.}  We start with the same latent for sampling and optimization, both running 100 steps, using empty prompts. The information flow (red arrows) differs only from the identity connection. However, the results of our attention distillation optimization (b) are clearly superior to sampling with KV-injection (a).}
    \label{fig:kvinjection}
\end{figure}

In this work, we propose a novel loss function to distill visual elements by reaggregating features within the self-attention mechanism; therefore, we refer to it as Attention Distillation (AD) loss. We leverage the UNet of the pretrained T2I diffusion model, Stable Diffusion~\cite{Rombach2021HighResolutionIS}, to extract image features from self-attention modules. As illustrated in Fig.~\ref{fig:method}~(a), we first reaggregate the visual information of the $KV$ features ($K_s$ and $V_s$) from the reference branch according to $Q$ from the target branch, which is the same as KV-injection. We regard this attention output as the \emph{ideal} stylization. Then, we calculate the attention output of the target branch and compute the L1 loss w.r.t. the ideal attention output, which defines the AD loss: %. We formulate AD loss as follows:
\begin{equation}
    \mathcal{L}_{\mathrm{AD}}=\|\mathrm{Self\text{-}Attn}(Q,K,V)-\mathrm{Self\text{-}Attn}(Q,K_s,V_s)\|_1.
\end{equation}

%Attention distillation optimization.
%\noindent{\textbf{Understanding AD loss.}} 
We can use the proposed AD loss to optimize a random latent noise via gradient descent, resulting in vivid texture or style reproduction in the output; see Fig.~\ref{fig:kvinjection}~(b) for example. This can be attributed to the backpropagation in optimization, which allows information to flow not only across the (\textit{residual}) self-attention modules but also through the identity connection. With continuous optimization, the gap between $Q$ and $K_s$ gradually narrows, making attention more and more accurate, and eventually, features are correctly aggregated to produce the desired visual details.

Following recent experimental analysis~\cite{cao2023masactrl, pnpDiffusion2022, jeong2024visual}, we empirically select the last 6 self-attention layers of the UNet to compute AD loss. Additionally, during optimization, we simulate the sampling process of diffusion models by linearly decreasing the timestep $t$ input to the UNet from $T$ to $0$. We begin with different random latent noises and optimize them over 100 steps. Note that during the whole optimization, the predicted noise from U-Net is totally discarded, and we continuously update the same latent.

To better understand our AD loss, we present the optimization results across multiple runs, as shown in Fig.~\ref{fig:multipleruns}. These results demonstrate that: i) AD loss effectively distills high-quality visual characteristics in style and texture; ii) AD loss is self-adapted to different spatial structures, showcasing diversity across multiple runs.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/multipleruns.pdf} 
    \vspace*{-1mm}
    \caption{\textbf{Optimizing attention distillation loss across multiple runs.} The coherence in texture and style, and the variations in structure across multiple runs of the same reference, demonstrates the ability of our AD loss in style alignment and spatial adaption.}
    \label{fig:multipleruns}
\end{figure}


\subsection{Content-preserving Optimization}
\label{sec:method_optim}
With the texture and style distilled by AD loss, we can further align the synthesized content to another reference image using a content loss. Such optimization allows the synthesis of images that transform the visual elements of one image while preserving the target content, achieving tasks such as style transfer, appearance transfer, and more.

As illustrated in Fig.~\ref{fig:method}~(b), we define the content loss similarly to AD loss, which is also based on the self-attention mechanism, fully drawing the advantage of the deep understanding of images in diffusion models. In particular, the L1 loss computed between the target queries $Q$ and the reference queries $Q_c$, formulates the content loss: 
\begin{equation}
    \mathcal{L}_{\mathrm{content}}=\|Q-Q_c\|_1.
\label{eq:content}
\end{equation}
In implementation, we also select the last 6 self-attention layers to compute the content loss, consistent with AD loss. The objective of content-preserving optimization is:
\begin{equation}
\mathcal{L}_{\mathrm{total}}=\mathcal{L}_{\mathrm{AD}}+\lambda\mathcal{L}_{\mathrm{content}}.
\end{equation}
After optimization, the optimized latent code is decoded into image space using the pretrained VAE. We have summarized the content-preserving optimization in Algorithm 1 of the supplementary material.



\subsection{Attention Distillation Guided Sampling}
\label{sec:method_sampling}
The syntheses above are using backpropagation optimization. In this section, we introduce how we incorporate attention distillation loss into the sampling process of diffusion models in an improved Classifier Guidance manner.
%as an improved Classifier Guidance.

According to~\cite{dhariwal2021beatgans}, Classifier Guidance alters the denoising direction during the denoising process, thereby generating samples from $p(z_t|c)$, which can be formulated as:  % the update direction is modified as
\begin{equation}
    \hat{\epsilon}_\theta=\epsilon_\theta(z_t, t, y)-\alpha\sigma_t\nabla_{z_t}\log p(c|z_t),
    \label{eq:noise_update}
\end{equation}
where $t$ is the timestep, $y$ denotes the prompts, and $\epsilon_\theta$ and $z_t$ refer to the denoising network and the latent in LDM, respectively. $\alpha$ controls the guidance strength. Inspired by~\cite{epstein2023selfguidance}, we guide the diffusion sampling process using an energy function based on attention distillation loss.
%can be incorporated as guidance into the diffusion sampling process.
%instead of relying solely on classifier probabilities, 

Specifically, during DDIM sampling~\cite{song2021ddim}, the latent $z_t$ at timestep $t$ are translated to $z_{t-1}$ according to the update direction $\epsilon_\theta$ estimated from the denoising network:
\begin{equation}
    z_{t-1}=\sqrt{\bar{\alpha}_{t-1}}\hat{z}_0+\sqrt{1-\bar{\alpha}_{t-1}}\epsilon_\theta,
    \label{eq:sampling}
\end{equation}
where $\hat{z}_0=\frac{z_t-\sqrt{1-\bar{\alpha}_t}\epsilon _\theta}{\sqrt{\bar{\alpha}_t}}$. Replace $\epsilon_\theta$ with $\hat{\epsilon}_\theta$ from Eq.~\eqref{eq:noise_update}:
%By replacing $\epsilon_\theta$ in Eq.~\ref{eq:sampling} with $\hat{\epsilon}_\theta$ from Eq.~\ref{eq:noise_update}, we get:
\begin{equation}
    z_{t-1}=\underbrace{\sqrt{\bar{\alpha}_{t-1}}\hat{z}_0+\sqrt{1-\bar{\alpha}_{t-1}}\epsilon_\theta}_{\mathrm{DDIM\ Sampling}}+\alpha C\cdot\nabla_{z_t}\log{p(c|z_t)},
\end{equation}
where $C$ is a constant related to $t$. We define the energy function using our AD loss by substituting $\nabla_{z_t}\log{p(c|z_t)}$ with $\nabla_{z_t}\mathcal{L}_{AD}$. However, we found configuring the guidance strength is tricky; see Sec.~\ref{sec:exp} for detailed experimental analysis. To address this issue, we introduce an Adam optimizer~\cite{adam2015} to automatically manage the strength and compute gradients. For simplification, we approximate the term $\nabla_{z_t}\mathcal{L}_{AD}$ by $\nabla_{z_{t-1}}\mathcal{L}_{AD}$, enabling an initial DDIM sampling for $z_{t-1}$, followed by a straightforward optimization update. The AD loss takes as inputs the latent $z_{t-1}$ and the noise-disturbed reference latent $z_{t-1}^{ref}$, as illustrated in Fig.~\ref{fig:method}~(c). We update $z_{t-1}$ via AD loss optimization as:
\begin{equation}
    z_{t-1}:=z_{t-1}-\alpha C\cdot\nabla_{z_{t-1}}\mathcal{L}_{\mathrm{AD}}(z_{t-1},z_{t-1}^{ref}).
\end{equation}

With the guidance from AD loss, we can compute the losses on the latents with timestep conditioning, rather than converting the latent to image space and calculating image-level losses, as done in recent works~\cite{rout2024rbmodulation, liu2023more, bansal2024universal}. Using the Adam optimizer also enables us to establish a universal learning rate, alleviating the challenge of setting the guidance strength. The attention distillation guided sampling is detailed in Algorithm 2 of the supplementary. Note that the content loss proposed in Eq.~\eqref{eq:content} can also be added into the sampling process working with AD loss, further to preserve the structure of a content reference image.

% where $C$ is a constant. For convenience, we approximate the term $\nabla_{z_t}\log{p(c|z_t)}$ by $\nabla_{z_{t-1}}\log{p(c|z_{t-1})}$, allowing us to update $z_{t-1}$ in a simpler optimization manner. We define the energy function using our AD loss, which takes as inputs the latent $z_{t-1}$ and the noise-disturbed reference latent $z_{t-1}^{ref}$, and then computes the AD loss, as illustrated in Fig.~\ref{fig:method}~(c). By optimizing AD loss, we now update $z_{t-1}$ as:
% \begin{equation}
%     z_{t-1}:=z_{t-1}-\alpha C\cdot\nabla_{z_{t-1}}\mathcal{L}_{\mathrm{AD}}(z_{t-1},z_{t-1}^{ref}).
% \end{equation}

% With such guidance from AD loss, we can compute the losses directly on the latent with timestep conditioning, rather than converting the latent to image space and calculating image-level losses, as done in recent works~\cite{rout2024rbmodulation, liu2023more, bansal2024universal}. However, we experimentally found that configuring the guidance scale is tricky. To address this issue, we introduce an Adam optimizer~\cite{adam2015} to manage the scale and compute gradients automatically. We can easily establish a universal learning rate thanks to Adam optimizer, mitigating the above challenge. See Sec.~\ref{sec:exp} for further experimental analysis. We have also summarized the attention distillation guided sampling in Algorithm 2 of the supplementary.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/vae.pdf} 
    \vspace*{-1mm}
    \caption{\textbf{Improved VAE decoding.} The pretrained VAE is lossy in high-frequency details. Fine-tuning the VAE with the reference image over several steps (denoted as VAE*) can enhance the reconstruction quality and the decoding for novel image synthesis.} %, leading to upper-bounded decoded results
    \label{fig:vae}
\end{figure}



\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/transfer.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{Comparisons of style and appearance transfer.} Our comparisons primarily focus on recent diffusion-based methods of style and appearance transfer, including CSGO~\cite{xing2024csgo}, StyleShot~\cite{gao2024styleshot}, StyleID~\cite{chung2024styleid}, and Cross-Image Attention~\cite{alaluf2024cross}. Additionally, we include traditional methods such as NST~\cite{gaty2016styletransfer} and transformer-based methods such as StyTR$2$~\cite{Deng_Tang_Dong_Ma_Pan_Wang_Xu_2022} and SpliceViT~\cite{Tumanyan_Bar-Tal_Bagon_Dekel_2022} for comparison.}
    \label{fig:transfer}
\end{figure*}
%Our comparisons primarily focus on  style and appearance transfer for comparison


\subsection{Improved VAE Decoding}
Experimental evidence~\cite{zhu2023designing, avrahami2023blendedlatent} suggests that the VAE employed in latent diffusion models is perceptually lossy. For tasks that require high-frequency local details, such as texture synthesis, we can \emph{optionally} fine-tune the weights $\theta$ of the VAE decoder $\mathcal{D}(\cdot)$ on the example image $x$ to enhance its reconstruction quality using L1 loss, following~\cite{avrahami2023blendedlatent}:
\begin{equation}
    \theta^*=\mathrm{arg}\min_{\theta}\|\mathcal{D}_\theta(\mathcal{E}(x))-x\|_1,
\end{equation}
where $\mathcal{E}(\cdot)$ denotes the VAE encoder. Fig.~\ref{fig:vae} presents some results of the reconstruction and sampling, showing improved perceptual quality with the fine-tuned VAE.




% \section{Applications}


 % \subsection{Preliminaries: Latent Diffusion Model and KV-Injcetion}
% Recently, diffusion models have achieved state-of-the-art results in the field of image generation due to their robust capability to model complex data distributions. In particular, latent diffusion models(LDM), a.k.a Stable Diffusion , utilize a powerful pre-trained autoencoder to compress images into a latent space for training denoising network, significantly reducing the computational cost of training and sampling. Specifically, given an image $x\in\mathbb{R}^{H\times W\times3}$ in RGB space, the encoder $E$ encodes $x$ into a latent representation $z=E(x)$, and the decoder $D$ reconstructs the image from the latent representation, yielding $\tilde{x}=D(z)=D(E(x))$, where $z\in\mathbb{R}^{h\times w\times c}.$ The training objective of denoising network is defined as:
% $$L_{LDM}:=\mathbb{E}_{\mathcal{E}(x),y,\epsilon\sim\mathcal{N}(0,1),t}\bigg[\|\epsilon-\epsilon_\theta(z_t,t,y)\|_2^2\bigg]$$

% Notably, the denoising network $\epsilon_\theta$ consists of a series of Residual Block, Self Attention and Cross Attention modules, all of which are integrated within the prediction branch of the residual network.
% \begin{figure}[ht]
% \centering
% \includegraphics[scale=0.15]{figs/layers.png} 
% \caption{Method}
% % \label{fig01}
% \end{figure}

% The U-Net denoising network captures long-range dependencies among data using self-attention and incorporates general conditioning inputs, such as text or bounding boxes, through cross-attention. The formula for the attention mechanism is as follows:
% $$\text{Attention}(Q,K,V)=\text{Softmax}(\frac{QK^T}{\sqrt{d}})V$$
% The core of the attention mechanism is centered on calculating the weight matrix based on the similarity between queries (Q) and keys (K), followed by performing a weighted aggregation of values (V). Recent studies have demonstrated that values derived from the self-attention module contain rich image information, encompassing both global structures and local texture details. Tune-A-Video utilizes self-attention across batches to generate similar image content. MasaCtrl proposes a mask-guided mutual self-attention strategy that facilitates text-based non-rigid image synthesis and real image editing without the need for fine-tuning. This technique, known as KV Injection, has quickly been applied to various tasks such as image translation, style transfer, texture synthesis, and even 3D composition to maintain visual consistency. The essence of KV-Injection lies in modifying self-attention to implement cross-attention between images, leveraging the attention formula to re-aggregate visual information from reference images according to new queries generated from synthesized images. However, these methods are influenced by factors such as the residual mechanism, preventing them from fully realizing the potential of KV-Injection.

% \begin{figure}[ht]
% \centering
% \includegraphics[scale=0.5]{figs/0.jpg} 
% \caption{Method}
% \label{fig01}
% \end{figure}

% We leverage the U-Net of the SD model to extract features from images in the self-attention module. The $Q$ from the generated images and the $K_s$ and values $V_s$ from the style or texture image are processed through the attention formula to obtain the output. Based on the previous works, this process $\text{Attention}(Q,K_s,V_s)$ re-aggregates the visual information of the style image according to the $Q$ of the generated image. The output can represent an ideal stylized result, while the original $\text{Attention}(Q,K,V)$ computation yields an unstyled result. We define the L1 distance between the two as the style loss, $L_{style}$, and optimize the generated image using gradient descent. Because this method simultaneously calculates the differences between different layers, there is no error accumulation, thus reducing the impact of query errors from a specific layer. By updating the generated results through backpropagation, the process is direct and thorough. Continuous optimization gradually reduces the gap between $Q$ and $K_s$, making the attention increasingly accurate, ultimately aggregating to produce the desired visual effect.\par
% $$L_{style}=||\text{Attention}(Q,K,V)-\text{Attention}(Q,K_{s},V_{s})||_1$$
% \subsection{Content Loss}
% The style/texture transfer tasks require maintaining the semantic structure of the content image. P2P, PhotoSwap, and Pix2Pix-Zero utilize self-attention and cross-attention maps to preserve the structure of images.  PnP uses the method of injecting convolutional features to preserve the layout of the image. StyldID proposes query preservation techniques to maintain the original content.  We found that the querys from self-attention contain spatial information (visualization). Therefore, we define the L1 distance between the generated image's $Q$ and the content image's $Q_c$ as the content loss, $L_{content}$. 
% $$L_{content}=||Q-Q_c||_1$$
% The final loss is:
% $$L = L_{style} + \lambda L_{content}$$

% \subsection{Masked Attention Distillation Loss}
% To address the issue of foreground-background confusion, MasaCtrl proposed a mask-guided KV-injection approach, enabling Q to query specified regions based on a mask, thereby alleviating inaccuracies in querying. Inspired by this, we introduce the incorporation of mask guidance when calculating the attention distillation loss, thereby constraining the values queried by Q. Specifically, given an input reference image $x_s\in\mathbb{R}^{h\times w\times 3}$, its corresponding source segmentation map $S_s\in\mathbb{R}^{h\times w\times 1}$, and the target segmentation map $S_t\in\mathbb{R}^{h'\times w'\times 1}$, we first flatten Ss and St , downsample them to match the resolution of Q and K, resulting in $\bar{S_s}$ and $\bar{S_t}$ . Subsequently, we compute the guiding mask $M$; with this mask, we can control the visual information aggregated by Q during attention computation to focus solely on the corresponding regions:
% $$M^*=S_s - S_t^T$$
% $$ M:= 
% \begin{cases} 
% \text{True} & \text{if } M^* > 0 \\ 
% \text{False} & \text{otherwise} 
% \end{cases}$$
% $$\mathcal{L}_{\mathrm{MAD}}=||\mathrm{Self\text{-}Attn}(Q,K,V)-\mathrm{Self\text{-}Attn}(Q,K_{s},V_{s};M)||_{1}$$

% \subsection{Optimized VAE Reconstruction}
% The previous discussion indicates that SD employs VAE for image compression and reconstruction. Experimental evidence suggests that this method is lossy, leading to noticeable visual artifacts in certain textures. Inspired by the Blended Latent Diffusion work, we fine-tune the weights $\theta$ of the decoder on the reference image to enhance reconstruction quality.
% $$\theta^{*}=\underset{\theta}{\mathrm{argmin}}\|D_{\theta}(E\left(x\right)-x\|_1$$
% In our approach, the optimized VAE reconstruction is optional. It is only necessary in instances where the texture comprises perceptually significant fine details.
% \begin{figure}[ht]
% \centering
% \includegraphics[scale=0.3]{figs/VAE.png} 
% \caption{Method}
% \label{fig01}
% \end{figure}
% \subsection{Improved Classifier Guidance}
% \begin{equation}
% \hat{\epsilon}=\epsilon_\theta(x_t)-\sqrt{1-\alpha_t}\nabla_{x_t}\log p_\phi(y|x_t)
% \end{equation}

% \begin{equation}
% x_{t-1}=\sqrt{\alpha_{t-1}}\left(\frac{x_t-\sqrt{1-\alpha_t}\hat{\epsilon}}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t-1}}\hat{\epsilon}
% \end{equation}
% \par
% In BEATS GAN, the classifier guidance method was proposed, which uses gradients from a classifier to guide generation. Subsequently, many works have introduced various models into the sampling process of diffusion models to achieve controlled generation effects. We attempted to use this method to calculate gradients for guiding generation based on our proposed loss function. However, during the experiments, we found it difficult to find an ideal guidance scale when the number of sampling steps was small, and different textures/styles required searching for different guidance scales. The Universal Guidance for Diffusion Models proposed a repetitive iterative approach to alleviate this issue.However, their method uses the decoder to decode latent, inputting the model's predicted images, which is often inaccurate and over-consumption of computing resources. Here, we present a simpler and more effective solution to address this problem.
% %我们的优势是不需要训练额外的分类器，借助Unet自身，在潜空间计算损失.\par

%  \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.3]{figs/1.jpg} 
% \caption{Method}
% \label{fig02}
% \end{figure}
%  \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.3]{figs/2.jpg} 
% \caption{Method}
% \label{fig03}
% \end{figure}

% By substituting Equation (1) into Equation (2), we can rewrite it in the following form:


% \begin{align}
% \begin{split}
% x_{t-1}=&\sqrt{\alpha_{t-1}}\left(\frac{x_t-\sqrt{1-\alpha_t}\epsilon_\theta(x_t)}{\sqrt{\alpha_t}}\right)+ \\
% &\sqrt{1-\alpha_{t-1}}\epsilon_\theta(x_t)+C\nabla_{x_t}\log p_\phi(y|x_t)
% \end{split}
% \end{align}

% where, $\sqrt{\alpha_{t-1}}\left(\frac{x_t-\sqrt{1-\alpha_t}\epsilon_\theta(x_t)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t-1}}\epsilon_\theta(x_t)$ is the original DDIM sampling result. $C=\left(\frac{(1-\alpha_t)-\sqrt{\alpha_t}\sqrt{1-\alpha_t}}{\sqrt{\alpha_t}}\right)\sqrt{1-\alpha_{t-1}}$.

% It is observed that the essence of this method is to update the latent values based on gradients, and we can fully utilize existing optimizers to manage the step size and direction of the updates. Below are the results using the Adam optimizer, with a fixed learning rate and 50 sampling steps, optimizing for a different number of iterations at each time step.
%  \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.5]{figs/3.jpg} 
% \caption{Method}
% \label{fig04}
% \end{figure}

% With the help of optimizer, we can easily find a universal learning rate, avoiding the issues mentioned above. By sampling just 50 steps and performing three optimization iterations at each step, we can achieve very good results. This significantly increases the synthesis speed compared to pure optimization solutions.
% \par
% Our approach can seamlessly integrate with Classifier-free Guidance, allowing us to control the content of image generation through text prompts or by using additional networks like ControlNet and IP-Adapter for image prompts and using MultiDiffusion for arbitrary resolution texture synthesis.


%  \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.3]{figs/4.jpg} 
% \caption{Method}
% \label{fig05}
% \end{figure}

\label{sec:method}



==> sec/4_exp.tex <==

% \begin{figure*}[htp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/transfer.pdf} 
%     \caption{\textbf{Comparisons of style and appearance transfer.} Our comparisons primarily focus on recent diffusion-based methods for both style and appearance transfer. Additionally, we include traditional methods, \ie NST~\cite{gaty2016styletransfer}, StyTR$^2$~\cite{Deng_Tang_Dong_Ma_Pan_Wang_Xu_2022} and SpliceViT~\cite{Tumanyan_Bar-Tal_Bagon_Dekel_2022} for comparison.}
%     \label{fig:transfer}
% \end{figure*}

\section{Experiments}
\label{sec:exp}

\subsection{Applications and Comparisons}
In the following, we apply our attention distillation loss to various visual characteristic transfer tasks and compare the results to state-of-the-art methods in each application. See the supplementary materials for detailed parameter configurations, running time, and additional results.

\vspace*{-3mm}
\paragraph{Style and Appearance Transfer.}
Following the spirit of the prominent work of Gatys \etal~\cite{gaty2016styletransfer}, we achieve style and appearance transfer through the optimization method described in Sec.~\ref{sec:method_optim}.
%In style and appearance transfer, the goal is to translate the style or appearance of a \yang{reference} image onto a \yang{content/structure} image. %Building on the landmark approach introduced by 
 %we alter the Gram loss to our AD loss, 
%we achieve this transfer through the optimization method described in Sec.~\ref{sec:method_optim}. 
We compare our method to CSGO~\cite{xing2024csgo}, StyleShot~\cite{gao2024styleshot}, StyleID~\cite{chung2024styleid}, StyTR$^2$~\cite{Deng_Tang_Dong_Ma_Pan_Wang_Xu_2022} and NST~\cite{gaty2016styletransfer} for style transfer, as well as Cross-Image Attention~\cite{alaluf2024cross} and SpliceViT~\cite{Tumanyan_Bar-Tal_Bagon_Dekel_2022} for appearance transfer. Fig.~\ref{fig:transfer} presents the qualitative comparison results. In style transfer, our method effectively captures high-quality, coherent style characteristics while simultaneously preserving the semantic structures of the content image. This is particularly evident in the sketch styles in the 3rd and 4th rows. In contrast, baseline methods exhibit notable style discrepancies, despite retaining the original structure. In appearance transfer, our method also shows superiority, avoiding the oversaturation of color seen in Cross-image Attention.


\vspace*{-3mm}
\paragraph{Style-specific Text-to-Image Generation.}

\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/stylet2i.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{Comparisons of style-specific text-to-image generation.} We compare our approach to InstantStyle~\cite{wang2024instantstyle}, Visual Style Prompting~\cite{jeong2024visual}, and RB-Modulation~\cite{rout2024rbmodulation} using three style references as examples. For each style, we utilize the same text prompts: ``\textit{A deer}'' (left), ``\textit{A rocket}'' (top right), and ``\textit{A piano}'' (bottom right).}
    \label{fig:stylet2i}
\end{figure*}

\begin{figure}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/controlnet.pdf} 
    \caption{By combining attention distillation guided sampling with ControlNet~\cite{zhang2023controlnet} into the text-to-image pipeline, we can produce high-quality results that align the structure with the condition image while maintaining style coherence with the style reference. }
    \label{fig:controlnet}
\end{figure}


%Generating images that integrate textual prompts with the specific artistic style of a reference image has gained popularity in art creation. To achieve this, we build on a text-to-image diffusion model, \ie Stable Diffusion, applying our AD loss within the diffusion sampling process as described in Sec.~\ref{sec:method_sampling}. 
As described in Sec.~\ref{sec:method_sampling}, we can apply our AD loss within the diffusion sampling, thereby realizing style-specific text-to-image generation. We set the reference as the desired style image. Fig.~\ref{fig:stylet2i} showcases some generated results, along with a comparison to alternative methods, including Visual Style Prompting~\cite{jeong2024visual}, InstantStyle~\cite{wang2024instantstyle}, and RB-Modulation~\cite{rout2024rbmodulation}. The results in Fig.~\ref{fig:stylet2i} demonstrate that our method aligns textual semantics comparably to existing methods while achieving notably better style coherence with the reference.

In addition to the above approach, we further incorporate ControlNet~\cite{zhang2023controlnet} to enable style-specific text-to-image generation with additional conditioning on various modalities, \eg depth and canny edges. Fig.~\ref{fig:controlnet} presents some generated examples. More results can be seen in the supplementary.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/ctrltex.pdf} 
%     \caption{\textbf{Comparisons of controlled texture synthesis.} \yang{Left: annotation control; Right: layout control.}}
%     \label{fig:control_tex}
% \end{figure}


% \zichong{
% \paragraph{Controlled Texture Synthesis.} The task here is to synthesize texture images 

% }

%Texture synthesis with spatial control is a challenging task, as existing methods often struggle to balance texture quality and spatial alignment. 
%In this work, we employ segmentation maps to guide the spatial structure of textures. 
\vspace*{-3mm}
\paragraph{Controlled Texture Synthesis.}
Our method can be applied to texture optimization as demonstrated in Sec.~\ref{sec:method_ADL}. Inspired by~\cite{cao2023masactrl}, we further incorporate mask guidance when calculating attention distillation loss, thereby constraining the values queried by $Q$, resulting in controlled texture synthesis. Specifically, given a source texture $x_s\in\mathbb{R}^{h\times w\times 3}$, its corresponding source segmentation map $S^s\in\mathbb{R}^{h\times w\times 1}$, and the target segmentation map $S^t\in\mathbb{R}^{h'\times w'\times 1}$, we first flatten $S^s$ and $S^t$ and downsample them to match the resolution of attention features, resulting in $\bar{S^s}$ and $\bar{S^t}$. Then, we compute the guiding mask $M$; with this mask, we restrict the visual information aggregated by $Q$ in attention computation to focus solely on the corresponding regions:

% $$M^*=S_s - S_t^T$$
\begin{equation}
 M_{i,j}:= 
\begin{cases} 
\text{True} & \text{if } \bar{S^s_i} = \bar{S^t_j} \\ 
\text{False} & \text{otherwise} 
\end{cases}   
\end{equation}
\begin{equation}
\mathcal{L}_{\mathrm{MAD}}=||\mathrm{Self\text{-}Attn}(Q,K,V)-\mathrm{Self\text{-}Attn}(Q,K_{s},V_{s};M)||_{1}
\end{equation}

%provided by the user
To further ensure the alignment with the target mask, we fill the target mask as initialization with pixels randomly drawn from corresponding labeled regions of the source image. Then, we regard this init as the content reference and add a content loss as Sec.~\ref{sec:method_optim} based on the query features.
%Combined with content loss from Q, we can achieve refined texture details and spatial alignment through optimization method. 
Figs.~\ref{fig:teaser} and~\ref{fig:control_tex} present our controlled texture synthesis results. Compared to GCD~\cite{zhou2023neural}, a patch-based neural texture optimization method, our results exhibit comparable texture details with smoother object edges. In contrast, GCD suffers from artifacts of color aliasing; see the 2nd row of Fig.~\ref{fig:control_tex}.

Recently, Self-Rectification~\cite{zhou2024generating} introduced a ``lazy-editing'' control for generating non-stationary textures. Aiming at the same goal, we utilize SDEdit~\cite{meng2022sdedit} to preserve the structure of the layout image edited by the user. Then, we incorporate our proposed AD loss and content loss into the sampling (as Sec.~\ref{sec:method_sampling}). As compared in Fig.~\ref{fig:control_tex}, Self-Rectification outputs smoother texture transitions, while our results better adhere to the original texture examples.
% \paragraph{Masked Attention Distillation Loss.} , effectively addressing this issue
% To address the issue of foreground-background confusion, MasaCtrl proposed a mask-guided KV-injection approach, enabling Q to query specified regions based on a mask, thereby alleviating inaccuracies in querying. Inspired by this, we introduce the incorporation of mask guidance when calculating the attention distillation loss, thereby constraining the values queried by Q. Specifically, given an input reference image $x_s\in\mathbb{R}^{h\times w\times 3}$, its corresponding source segmentation map $S^s\in\mathbb{R}^{h\times w\times 1}$, and the target segmentation map $S^t\in\mathbb{R}^{h'\times w'\times 1}$, we first flatten $S^s$ and $S^t$ , downsample them to match the resolution of Q and K, resulting in $\bar{S^s}$ and $\bar{S^t}$ . Subsequently, we compute the guiding mask $M$; with this mask, we can control the visual information aggregated by Q during attention computation to focus solely on the corresponding regions:
% % $$M^*=S_s - S_t^T$$
% $$ M_{i,j}:= 
% \begin{cases} 
% \text{True} & \text{if } \bar{S^s_i} = \bar{S^t_j} \\ 
% \text{False} & \text{otherwise} 
% \end{cases}$$
% $$\mathcal{L}_{\mathrm{MAD}}=||\mathrm{Self\text{-}Attn}(Q,K,V)-\mathrm{Self\text{-}Attn}(Q,K_{s},V_{s};M)||_{1}$$

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/ctrltex.pdf} 
    \caption{\textbf{Comparisons of controlled texture synthesis.} Left: annotation control; Right: layout control.}
    \label{fig:control_tex}
\end{figure}


\vspace*{-3mm}
\paragraph{Texture Expansion.}
It is very difficult to synthesize ultra-high resolution textures using traditional methods, given the limited patch sources. Here, we apply our attention distillation guided sampling to the MultiDiffusion~\cite{bar2023multidiffusion} model, enabling texture expansion to arbitrary resolution.
%Traditional texture synthesis methods are often constrained by computational resources, limiting the generation of ultra-high-resolution textures and increasing the likelihood of artifacts. 
Although SD-1.5~\cite{Rombach2021HighResolutionIS} is trained on images of size 512$\times$512, surprisingly, it demonstrates robust capabilities in large-size texture synthesis when incorporating attention distillation. Fig.~\ref{fig:texexp} presents comparisons of texture expansion to size 512$\times$1536 with GCD~\cite{zhou2023neural} and GPDM~\cite{elnekave2022generating}. Our approach shows significant advantages in such a challenging task. %See supplementary for more results.}

\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/texexp.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{Comparisons of texture expansion.} Taking a 512$\times$512 texture image as the input example, we expand it with automatic semantic understanding and synthesize results at the resolution 512$\times$1536. We compare our approach with GCD~\cite{zhou2023neural} and GPDM~\cite{elnekave2022generating}.}
    \label{fig:texexp}
\end{figure*}



\subsection{Ablation Studies}

\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/abl_content_loss.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{Ablation of content loss weights.} Varying the content loss weights $\lambda$ on two examples, one each for style transfer (left) and appearance transfer (right). The results demonstrate how the content loss helps preserve the source image content during the transfer. When the weights are within an appropriate range, the results exhibit varying levels of abstraction and appearance transition.}
    \label{fig:abl_closs}
\end{figure*}

\begin{figure}[htp]
    \centering
    \vspace*{-2mm}
    \includegraphics[width=1.0\linewidth]{figs/abl_optim1.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{Impact of the optimizer for managing guidance strength.} Both cases--with and without the Adam optimizer~\cite{adam2015}--were conducted with 50 diffusion sampling steps. All results are generated using Stable Diffusion v1.5~\cite{Rombach2021HighResolutionIS}, with empty text prompts. The learning rate of the Adam optimizer is set to 0.02.}%, and we performed two optimization iterations after each sampling step.} the introduction of
    \label{fig:abl_optim}
\end{figure}

In this section, we present ablation study results on two aspects of our approach: i) the impact of content loss weight in content-preserving optimization (Sec.~\ref{sec:method_optim}), and ii) the optimizer for managing guidance strength in attention distillation guided sampling (Sec.~\ref{sec:method_sampling}).

\vspace*{-3mm}
\paragraph{Content loss weight.} As shown in Fig.~\ref{fig:abl_closs}, varying the content loss weight $\lambda$ brings intriguing effects on the transfer results. In style transfer, for instance, the abstract style example shown on the left illustrates how the adjustment of $\lambda$ results in different levels of abstraction, offering flexibility for artistic creation. In appearance transfer, thanks to the precise semantic understanding from diffusion networks, the facial image transfer shown on the right exhibits a smooth identity transition along with the $\lambda$ varies.

\vspace*{-3mm}
\paragraph{Optimizer.} Fig.~\ref{fig:abl_optim} demonstrates the importance of the optimizer in managing guidance strength. We experimentally test a naive strategy of manually setting the guidance strength to control the scale of gradient updates to the latents. However, varying this strength manually often fails to yield reasonable results: textures or appearance features in the examples are typically lost, as shown in the last three columns of Fig.~\ref{fig:abl_optim}. In contrast, introducing an Adam optimizer to manage latent optimization produces results that closely match the visual characteristics of the input examples (columns 2$\sim$4 in Fig.~\ref{fig:abl_optim}). Furthermore, increasing the number of optimization iterations within each timestep during sampling generally enhances the quality of generated results, although it also brings extra computation time. In practice, we set the iteration number to 2 to achieve an efficient balance, delivering high-quality results effectively.


\begin{figure}[t]
    \centering
    \vspace*{-3mm}
    \includegraphics[width=1.0\linewidth]{figs/userstudy.pdf} 
    \vspace*{-6mm}
    \caption{\textbf{User preference score.} We report the overall preference score comparing our method to selected alternatives across three transfer tasks. Each comparison is conducted individually, directly evaluating user preference between our results and those of each competing method. Note CIA stands for Cross-Image Attention~\cite{alaluf2024cross} and VSP as~\cite{jeong2024visual}. See supplementary for more details.}%\zichong{For brevity, CIA and VSP denote Cross-image Attention and Visual Style Prompting, respectively.}}% See supplementary for more details. }
    \label{fig:user}
\end{figure}

\subsection{User Preference Study}
To validate the qualitative analysis, we conduct a user study with 30 questions (5 questions for each of 6 selected competitors) on three transfer tasks. In each question, we showcase two results: one from our method and one from a competitor. The user was asked to choose the better one based on the provided instructions and criteria. We have collected 1500 responses from 50 participants, and the overall preference score is summarized in Fig.~\ref{fig:user}. Our method consistently outperforms the alternatives by significant margins. Please refer to the supplementary for more details.

% \begin{table}[htbp]%
%     \scriptsize 
%     \caption{
%     User preference score.
%     }
%     \label{tab:userstudy}
%     \vspace*{-5mm}
%     \begin{center}
%     \begin{tabular}{c|cc|cc|cc}
%       \hline
%       & \multicolumn{2}{c|}{\makecell[c]{Style Transfer}} & \multicolumn{2}{c|}{\makecell[c]{Appearance Transfer}} & \multicolumn{2}{c}{\makecell[c]{{ Style-specific} \\ {  Text-to-Image Generation}}}\\  \hline
%       \multirow{2}*{\makecell[c]{Ours\\ vs.}} & StyleID & StyTR$^2$ & CIA* & SpliceViT & InstantStyle & VSP* \\ \cline{2-7} %\hline
%       & 80.4\% & 83.2\% & 61.6\% & 88.0\% & 74.4\% & 83.2\% \\
%       \hline
%     \multicolumn{7}{l}{\scriptsize * CIA and VSP denote Cross-image Attention and Visual Style Prompting, respectively.}\\
%     \end{tabular} 
%     \end{center}
% \end{table}%





==> sec/5_con.tex <==
\section{Conclusion}
\label{sec:conclusion}

We have presented a unified approach for various visual characteristics transfer tasks, including style/appearance transfer, style-specific image generation, and texture synthesis. The key to the proposed method is a novel attention distillation loss, which calculates the difference between the ideal and current stylization, and gradually modifies the synthesis. Our method overcomes the limitations of previous works, and experiments have validated its superiority.%over existing methods.

